An Empirical Study of the Cost of DNS-over-HTTPS

DNS is a vital component for almost every networked application. Originally it was designed as an unencrypted protocol, making user security a concern. DNS-over-HTTPS (DoH) is the latest proposal to make name resolution more secure. In this paper we study the current DNS-over-HTTPS ecosystem, especially the cost of the additional security. We start by surveying the current DoH landscape by assessing standard compliance and supported features of public DoH servers. We then compare different transports for secure DNS, to highlight the improvements DoH makes over its predecessor, DNS-over-TLS (DoT). These improvements explain in part the significantly larger take-up of DoH in comparison to DoT. Finally, we quantify the overhead incurred by the additional layers of the DoH transport and their impact on web page load times. We find that these overheads only have limited impact on page load times, suggesting that it is possible to obtain the improved security of DoH with only marginal performance impact.

==> Makefile <==
SOURCE=*
TARGET=paper

all: $(TARGET).pdf


%.ps: %.dvi
	dvips $(@:.ps=.dvi)

%.pdf: %.tex $(SOURCE).tex $(SOURCE).bib
	#$(MAKE) -C graphs
	pdflatex $(@:.pdf=.tex)
	bibtex $(@:.pdf=.aux)
	pdflatex $(@:.pdf=.tex)
	pdflatex $(@:.pdf=.tex)

%.dvi: %.tex $(SOURCE).tex $(SOURCE).bib
	latex $(@:.dvi=.tex)
	bibtex $(@:.dvi=.aux)
	latex $(@:.dvi=.tex)
	latex $(@:.dvi=.tex)

clean:
	rm -f *.log *.blg *.bbl *.toc *.aux *.out *.lof *.lot *.ptc *.synctex.gz
	rm -f *.dvi *.pdf
	rm -f *~

count:
	texcount $(TARGET).tex -merge

spellcheck:
	for i in *.tex; do \
		aspell check --lang=en_US --mode=tex --home-dir=. --dont-backup $$i; \
	done

diff :
	./git-latexdiff --ignore-makefile --verbose --main $(TARGET).tex --output build/$(TARGET)_diff.pdf --exclude-textcmd="author" --config="PICTUREENV=(?:picture|DIFnomarkup|acks|CCSXML)[\w\d*@]*" 60e17c7b3833efdf82fa43a534e6a1ccf76f4c34 --

.PHONY: cr
cr:
	rm -rf cr/
	mkdir -p cr/
	latexpand --expand-bbl build/$(TARGET).bbl $(TARGET).tex > cr/main.tex
	mkdir -p cr/graph
	for fig in `pcregrep -o1 '\\includegraphics.*{(.*)}' cr/main.tex`; do \
		cp $$fig.* cr/graph/; \
	done
	COPYFILE_DISABLE=true tar -czf cr.tar.gz -C cr/ .


==> discussion.tex <==
\section{Discussion}

\paragraph{Head-of-line blocking.} 
In this paper we have discussed the impact of head-of-line blocking at the DNS resolver.
While the phenomenon of head-of-line blocking has already been discussed in the context of web performance, it is even more important for DNS.
In the typical web scenario, the browser maintains multiple TLS connections to every website, so that a slowdown on one of the connections most likely affects a single webpage only. Since the user's web browser holds the connection, only that user gets impacted.
In contrast, a DNS resolver typically multiplexes DNS requests from many sources: in the case of a resolver on a host, typically all DNS queries originating from this host. For a site-wide DNS resolver, this resolver would typically be responsible for DNS queries from all users on this site. In that case, a slowdown in DNS resolution does not affect a single user or application anymore, but it can potentially affect many users. Even worse, a slowdown caused by one user can affect all other users without any possible mitigation by them. We thus argue that in this scenario, the choice of the transport protocol is critical.

%\paragraph{The general case for transport protocols.}
%HTTP(s) nowadays is the single most important transport protocol in the Internet, with ever more information being sent over and more application relying on it.
%We argue that all considerations we discuss in this paper, do not only hold for DNS, but will likely be important whenever a protocol is to be wrapped into HTTP.
\begin{comment}
T: meh
\end{comment}

\paragraph{DDoS-resilience.} DNS via UDP is an exploitable protocol for distributed denial-of-service attacks~\cite{anagnostopoulos2013dns}. Indeed, UDP is particularly prone to IP source address spoofing, and DNS replies enable amplification attacks, as the responses can be much larger than the queries.
As a consequence, the IETF has demanded the root DNS servers to be over-provisioned, i.e., servers are required to be able to handle up to three time the normal query load~\cite{rfc2870}. Obviously, DNS-over-HTTP runs exclusively over TCP. Since source address spoofing on TCP is hardly possible, DNS-over-HTTP is not vulnerable to this type of DDoS attacks. This makes DoH an attractive choice for DNS server operators, in particular open resolvers, such as Cloudflare or Google, which are inherently more exposed to DDoS.

==> git-latexdiff <==
#! /bin/bash

# Main author: Matthieu Moy <Matthieu.Moy@imag.fr> (2012 - 2017)
# (See the Git history for other contributors)
#
# Copying and distribution of this file, with or without modification,
# are permitted in any medium without royalty provided the copyright
# notice and this notice are preserved.  This file is offered as-is,
# without any warranty.
#
# git-latexdiff is a wrapper around latexdiff
# (http://www.ctan.org/pkg/latexdiff) that allows using it to diff two
# revisions of a LaTeX file.
#
# The script internally checks out the full tree for the specified
# revisions, calls latexpand to flatten the document and then calls
# latexdiff-so (if available, otherwise latexdiff). Therefore,
# this works if the document is split into multiple .tex files.
#
# Try "git latexdiff -h" for more information.
#
# To install, just copy git-latexdiff in your $PATH.

# Missing features (patches welcome ;-):
# - diff the index
# - hardlink temporary checkouts as much as possible

# Alternatives:
#
# There is another script doing essentially the same here:
# https://github.com/cawka/latexdiff/blob/master/latexdiff-git
# My experience is that latexdiff-git is more buggy than
# git-latexdiff, but they probably just don't have the same bugs ;-)
#
# There are a bunch of other alternatives cited here:
#
#   http://tex.stackexchange.com/questions/1325/using-latexdiff-with-git
#
# Ideally, these scripts should be merged.

set -o errexit
set -o pipefail
set -o noclobber
# Used when symlinking files from the working tree: symlink .* files
# too.
shopt -s dotglob

# Some versions of git set $GIT_WORK_TREE when ran through an alias.
# This wouldn't work with git-latexdiff which plays with different
# work trees.
unset GIT_DIR
unset GIT_WORK_TREE

# (Comment and 'unset' line borrowed from Git's source code)
# Having this variable in your environment would break scripts because
# you would cause "cd" to be taken to unexpected places.  If you
# like CDPATH, define it for your interactive shell sessions without
# exporting it.
# But we protect ourselves from such a user mistake nevertheless.
unset CDPATH

# @GIT_LATEXDIFF_VERSION@ is substituted by the install script here,
# but not within git_latexdiff_compute_version().
git_latexdiff_version='@GIT_LATEXDIFF_VERSION@'

git_latexdiff_compute_version () {
    if [ "$git_latexdiff_version" = '@GIT_LATEXDIFF''_VERSION@' ]; then
	(cd "$(dirname "$0")" && git describe --tags HEAD 2>/dev/null || echo 'Unknown version')
    else
	echo "$git_latexdiff_version"
    fi
}

usage () {
    cat << EOF
Usage: $(basename "$0" | sed 's/git-/git /') [options] OLD [NEW]
       $(basename "$0" | sed 's/git-/git /') [options] OLD --
       $(basename "$0" | sed 's/git-/git /') [options] -- OLD
Call latexdiff on two Git revisions of a file.

OLD and NEW are Git revision identifiers. NEW defaults to HEAD.
If "--" is used for NEW, then diff against the working directory.

Options:
    --help                this help message
    --help-examples       show examples of usage
    --main <file>         name of the main LaTeX, R Sweave,
                            or Emacs Org mode file.
                            The search for the only file containing 'documentclass'
                            will be attempted, if not specified.
                            For non-LaTeX files, a reasonable \`prepare\` command
                            will be used unless explicitly provided
    --no-view             don't display the resulting PDF file
    --latex               run latex instead of pdflatex
    --bibtex, -b          run bibtex as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --biber               run BibLaTex-Biber as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --view                view the resulting PDF file
                            (default if -o is not used)
    --pdf-viewer <cmd>    use <cmd> to view the PDF file (default: \$PDFVIEWER)
    --no-cleanup          don't cleanup temp dir after running
    --no-flatten          don't call latexpand to flatten the document
    --cleanup MODE        Cleanup temporary files according to MODE:

                           - keeppdf (default): keep only the
                                  generated PDF file

                           - none: keep all temporary files
                                  (may eat your diskspace)

                           - all: erase all generated files.
                                  Problematic with --view when the
                                  viewer is e.g. evince, and doesn't
                                  like when the file being viewed is
                                  deleted.

    --latexmk             use latexmk
    --latexopt            pass additional options to latex (e.g. -shell-escape)
    -o <file>, --output <file>
                          copy resulting PDF into <file> (usually ending with .pdf)
                          Implies "--cleanup all"
    --tmpdirprefix        where temporary directory will be created (default: /tmp).
                            Relative path will use repository root as a base
    --verbose, -v         give more verbose output
    --quiet               redirect output from subprocesses to log files
    --prepare <cmd>       run <cmd> before latexdiff (e.g. run make to generate
                             included files)
    --ln-untracked        symlink uncommited files from the working directory
    --version             show git-latexdiff version.
    --subtree             checkout the tree at and below the main file
                             (enabled by default, disable with --whole-tree)
    --whole-tree          checkout the whole tree (contrast with --subtree)
    --ignore-latex-errors keep on going even if latex gives errors, so long as
                          a PDF file is produced
    --ignore-makefile     ignore the Makefile, build as though it doesn't exist
    -*                    other options are passed directly to latexdiff
    --bbl                 shortcut to flatten a bbl file of the same name as the project
    --latexpand OPT       pass option OPT to latexpand. Use multiple times like
                          --latexpand OPT1 --latexpand OPT2 to pass multiple options.
    --latexdiff-flatten   use --flatten from latexdiff instead of latexpand

Unrecognized options are passed unmodified to latexdiff.
EOF
}

examples () {
    cat <<EOF
Examples:

Pass --type=CHANGEBAR to latexdiff to get changebars in the margins
instead of red+trike/blue+underline diff:

    git latexdiff --type=CHANGEBAR HEAD^

Use a specific latexdiff configuration file:

    git latexdiff --config /path/to/file HEAD^
EOF
}

die () {
    echo "fatal: $*"
    exit 1
}

verbose () {
    if test "$verbose" = 1 ; then
	printf "%s ..." "$@"
    fi
}

verbose_progress () {
    if test "$verbose" = 1 ; then
	printf "."
    fi
}

verbose_done () {
    if test "$verbose" = 1 ; then
	echo " ${1:-done}."
    fi
}

verbose_say () {
    if test "$verbose" = 1 ; then
	printf "%s\n" "$@"
    fi
}

old=
new=
main=
view=maybe
cleanup=keeppdf
verbose=0
bibtex=0
biber=0
output=
initial_dir=$PWD
tmpdir_prefix="/tmp"
prepare_cmd=
flatten=1
subtree=1
uselatexmk=
latexopt=
ln_untracked=0
quiet=0
ignorelatexerrors=0
latexdiffopt=()
latexpand=()
bbl=0
latexdiff_flatten=0
latex=0


while test $# -ne 0; do
    case "$1" in
        "--help"|"-h")
            usage
            exit 0
            ;;
	"--help-examples")
	    examples
	    exit 0
	    ;;
	"--main")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    main=$1
	    ;;
	"--no-view")
	    view=0
	    ;;
	"--view")
	    view=1
	    ;;
	"--pdf-viewer")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    PDFVIEWER="$1"
	    ;;
	"--no-cleanup")
	    cleanup=none
	    ;;
	"--ignore-latex-errors")
	    ignorelatexerrors=1
	    ;;
        "--cleanup")
            shift
            case "$1" in
                "none"|"all"|"keeppdf")
                    cleanup="$1"
                    ;;
                *)
                    echo "Bad argument --cleanup $1"
                    usage
                    exit 1
                    ;;
            esac
            ;;
	"--no-flatten")
            flatten=0
            ;;
	"--ignore-makefile")
	    ignoremake=1
	    ;;
	"-o"|"--output")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    output=$1
	    cleanup=all
	    ;;
	"-b"|"--bibtex")
	    bibtex=1
	    ;;
	"--latex")
	    latex=1
	    ;;
	"--biber")
	    biber=1
	    ;;
	"--verbose"|"-v")
	    verbose=1
	    ;;
        "--quiet")
	    quiet=1
	    ;;
	"--version")
	    git_latexdiff_compute_version
            exit 0
	    ;;
	"--subtree")
	    subtree=1
	    ;;
	"--whole-tree")
	    subtree=0
	    ;;
	"--prepare")
	    shift
	    prepare_cmd="$1"
	    ;;
        "--latexmk")
            uselatexmk=1
            ;;
	"--latexpand")
	    shift
	    latexpand=("${latexpand[@]}" "$1")
	    ;;
	"--bbl")
	    bbl=1
	    ;;
	"--latexdiff-flatten")
	    latexdiff_flatten=1
            flatten=0
	    ;;
	"--latexopt")
	    shift
	    latexopt=$1
	    ;;
        "--ln-untracked")
            ln_untracked=1
            ;;
        "--no-ln-untracked")
            ln_untracked=0
            ;;
        "--tmpdirprefix")
	    shift
	    tmpdir_prefix="$1"
	    ;;
        -*)
            if test "$1" = "--" ; then
                if test -z "$new" ; then
                    new=$1
                else
                    echo "Bad argument $1"
                    usage
                    exit 1
                fi
            else
		case "$1" in
		    '--type'|'-t'|'--subtype'|'-s'|'--floattype'|'-f'|\
			'--config'|'-c'|'--preamble'|'-p'|'--encoding'|'-e'|\
			'--label'|'-L'|'--exclude-safecmd'|'-A'|\
			'--replace-safecmd'|'--append-safecmd'|'-a'|\
			'--exclude-textcmd'|'-X'|'--replace-textcmd'|\
			'--append-textcmd'|'-x'|'--replace-context1cmd'|\
			'--append-context1cmd'|'--replace-context2cmd'|\
			'--append-context2cmd'|'--packages'|'--math-markup'|\
			'--driver')
			# Options taking an immediate argument in
			# latexdiff => add both the option and its
			# argument.
			latexdiffopt+=("$1" "$2")
			shift
			;;
		    *)
			latexdiffopt+=("$1")
			;;
		esac
            fi
            ;;
        *)
	    if test -z "$1" ; then
		echo "Empty string not allowed as argument"
		usage
		exit 1
	    elif test -z "$old" ; then
		old=$1
	    elif test -z "$new" ; then
		new=$1
	    else
		echo "Bad argument $1"
		usage
		exit 1
	    fi
            ;;
    esac
    shift
done

initial_repo=$(git rev-parse --show-toplevel)

if test -z "$new" ; then
    new=HEAD
fi

if test -z "$old" ; then
    echo "fatal: Please, provide at least one revision to diff with."
    usage
    exit 1
fi

if test -z "$PDFVIEWER" ; then
    verbose "Auto-detecting PDF viewer"
    candidates="xdg-open evince okular xpdf acroread"
    if test "$(uname)" = Darwin ; then
        # open exists on GNU/Linux, but does not open PDFs
	candidates="open $candidates"
    fi

    for command in $candidates; do
	if command -v "$command" >/dev/null 2>&1; then
	    PDFVIEWER="$command"
	    break
	else
	    verbose_progress
	fi
    done
    verbose_done "$PDFVIEWER"
fi

case "$view" in
    maybe|1)
	if test -z "$PDFVIEWER" ; then
	    echo "warning: could not find a PDF viewer on your system."
	    echo "warning: Please set \$PDFVIEWER or use --pdf-viewer CMD."
	    PDFVIEWER=false
	fi
	;;
esac

if test $flatten = 1 &&
    ! command -v latexpand 2>/dev/null; then
    echo "Warning: latexpand not found. Falling back to latexdiff --flatten."
    latexdiff_flatten=1
    flatten=0
fi

if test $latex = 1; then
    LATEX_EXEC=latex
else
    LATEX_EXEC=pdflatex
fi

## end option parsing ##

check_knitr () {
    if test -z "$prepare_cmd"; then
	prepare_cmd="Rscript -e \"library(knitr); knit('$main')\""
    fi
    main="${main%\.*}.tex"
}

check_org () {
    if test -z "$prepare_cmd"; then
        prepare_cmd="emacs --batch --eval \"(load \\\"~/.emacs\\\")\" \"$main\" -f org-latex-export-to-latex --kill"
    fi
    main="${main%\.*}.tex"
}

log_cmd () {
    log=$1
    shift
    if [ "$quiet" = 1 ]; then
	"$@" >$log 2>&1
    else
	"$@"
    fi
}

# main is relative to initial_dir (if returned)
if test -z "$main" ; then
    printf "%s" "No --main provided, trying to guess ... "
    main=$(git grep -l '^[ \t]*\\documentclass')
    # May return multiple results, but if so the result won't be a file.
    if test -r "$main" ; then
	echo "Using $main as the main file."
    else
	if test -z "$main" ; then
	    echo "No candidate for main file."
	else
	    echo "Multiple candidates for main file:"
	    printf "%s\n" "$main" | sed 's/^/\t/'
	fi
	die "Please, provide a main file with --main FILE.tex."
    fi
fi

if test ! -r "$main" ; then
    die "Cannot read $main."
fi

ext=${main##*\.}
case "$ext" in
    Rnw) check_knitr ;;
    Rtex) check_knitr ;;
    org) check_org ;;
    *) ;;
esac

# Set LATEXDIFF_EXEC to either latexdiff or latexdiff-so. Prefer
# latexdiff-so if available.
if command -v latexdiff-so >/dev/null 2>&1; then
    LATEXDIFF_EXEC=latexdiff-so
elif command -v latexdiff >/dev/null 2>&1; then
    LATEXDIFF_EXEC=latexdiff
else
    die "latexdiff-so and latexdiff couldn't be found. Check your PATH."
fi
verbose_done "$LATEXDIFF_EXEC"

verbose "Creating temporary directories"

git_prefix=$(git rev-parse --show-prefix)
git_dir="$(git rev-parse --git-dir)" || die "Not a git repository?"
cd "$(git rev-parse --show-cdup)" || die "Can't cd back to repository root"
git_dir=$(cd "$git_dir"; pwd)
git_worktree=$(pwd)

# make main relative to git root directory
if test -n "$git_prefix" ; then
    main=$git_prefix$main
fi
mainbase=$(basename "$main" .tex)
maindir=$(dirname "$main")

tmpdir=$tmpdir_prefix/git-latexdiff.$$
mkdir "$tmpdir" || die "Cannot create temporary directory."

cd "$tmpdir" || die "Cannot cd to $tmpdir"
if test "$(uname -o 2>/dev/null)" = "Msys"; then
    tmpdir=$(pwd -W)
else
    tmpdir=$(pwd)
fi

mkdir old new || die "Cannot create old and new directories."

verbose_done
verbose_say "Temporary directories: $tmpdir/old and $tmpdir/new"
verbose "Checking out old and new version"

cd old || die "Cannot cd to old/"
if test "$ln_untracked" = 1; then
    (
	mkdir -p "$maindir" && cd "$maindir" &&
	    log_cmd ln-old.log ln -s "$initial_repo"/"$maindir"/* .
    ) || true
fi

if test "$subtree" = 1 && test -n "$git_prefix"; then
    checkoutroot=$git_prefix
else
    checkoutroot="."
fi

# Checkout a subtree, without touching the index ("git checkout" would)
(cd "$git_dir" && git archive --format=tar "$old" "$checkoutroot") | tar -xf -
# Also expand the possible submodules
(cd "$git_worktree" && git submodule foreach 'git archive --format=tar "$sha1" | tar -xf - --directory '$tmpdir/old'/$path')
verbose_progress
cd ../new || die "Cannot cd to new/"
if test "$new" == "--"; then
    # Copy working tree files
    (cd "$git_worktree" && git ls-files -- "$checkoutroot" | tar -cf - -T -) | tar -xf -
else
    # checkout new revision
    (cd "$git_dir" && git archive --format=tar "$new" "$checkoutroot") | tar -xf -
    (cd "$git_worktree" && git submodule foreach 'git archive --format=tar "$sha1" | tar -xf - --directory '$tmpdir/new'/$path')
fi
if test "$ln_untracked" = 1; then
    (
	mkdir -p "$maindir" && cd "$maindir" &&
	    log_cmd ln-new.log ln -s "$initial_repo"/"$maindir"/* .
    ) || true
fi

verbose_progress
cd ..

verbose_done

for dir in old new
do
    verbose "Running preparation command $prepare_cmd in $dir/$git_prefix"
    ( cd "$dir/$git_prefix/" && log_cmd prepare.log eval "$prepare_cmd" )
    if test ! -f "$dir/$main"; then
	die "$prepare_cmd did not produce $dir/$main."
    fi
    verbose_done
done

if [ "$ignorelatexerrors" = 1 ]; then
    latexopt="$latexopt -interaction=batchmode"
elif [ "$quiet" = 1 ]; then
    latexopt="$latexopt -interaction=nonstopmode"
else
    latexopt="$latexopt -interaction=errorstopmode"
fi

# Option to use latexdiff --flatten instead of latexpand
if test "$latexdiff_flatten" = 1; then
    latexdiffopt+=("--flatten")
fi

# Shortcut to include bbl
if test "$bbl" = 1; then
    bblexpand=("--expand-bbl" "$mainbase.bbl")
else
    bblexpand=()
fi

ignore_errors_maybe() {
    if [ "$compile_error" = 1 ] && [ "$ignorelatexerrors" = 1 ]; then
	echo "LaTeX errors were found - but attempting to carry on."
	compile_error=0
    fi
}

# Create flattened documents and keep for debugging
if test "$flatten" = 1; then
    if [ "$bbl" = 1 ]; then
	if [ ! -f "old/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing old/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd old/"$maindir"
	    log_cmd pdflatex0.log pdflatex $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    ignore_errors_maybe
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for old version"
	    fi
	fi
	if [ ! -f "new/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing new/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd new/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    ignore_errors_maybe
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for new version"
	    fi
	fi
    fi
    verbose "Running latexpand"
    (
	cd old/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > old-"$mainbase"-fl.tex \
	|| die "latexpand failed for old version"
    (
	cd new/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > new-"$mainbase"-fl.tex \
	|| die "latexpand failed for new version"
    verbose_done

    verbose "Running $LATEXDIFF_EXEC ${latexdiffopt[*]} old-${mainbase}-fl.tex new-${mainbase}-fl.tex > ./diff.tex"
    "$LATEXDIFF_EXEC" "${latexdiffopt[@]}" old-"$mainbase"-fl.tex new-"$mainbase"-fl.tex > diff.tex \
	|| die "$LATEXDIFF_EXEC failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new-"$mainbase"-fl.tex new-"$mainbase"-fl.tex.orig
    mv -f diff.tex new/"$main"
    verbose_done
else
    verbose "Running $LATEXDIFF_EXEC ${latexdiffopt[*]} old/$main new/$main > ./diff.tex"
    "$LATEXDIFF_EXEC" "${latexdiffopt[@]}" old/"$main" new/"$main" > diff.tex \
	|| die "$LATEXDIFF_EXEC failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main.orig"
    mv -f diff.tex new/"$main"
    verbose_done
fi

verbose "Compiling result"

compile_error=0
cd new/"$maindir" || die "Can't cd to new/$maindir"
if test -f Makefile && test "$ignoremake" != 1 ; then
    log_cmd make.log make || compile_error=1
elif test "$uselatexmk" = 1; then
    log_cmd latexmk.log latexmk -f -pdf -silent $latexopt "$mainbase" || compile_error=1
else
    log_cmd pdflatex1.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    if test "$bibtex" = 1 ; then
	log_cmd bibtex.log bibtex "$mainbase" || compile_error=1
    fi
    if test "$biber" = 1 ; then
	log_cmd biber.log biber "$mainbase" || compile_error=1
    fi
    log_cmd pdflatex2.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    log_cmd pdflatex3.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
fi

verbose_done

ignore_errors_maybe

if test $latex = 1; then
    dvips "$mainbase".dvi
    ps2pdf "$mainbase".ps
fi

pdffile="$mainbase".pdf
if test ! -r "$pdffile" ; then
    echo "No PDF file generated."
    compile_error=1
fi

if test ! -s "$pdffile" ; then
    echo "PDF file generated is empty."
    compile_error=1
fi

if test "$compile_error" = "1" ; then
    echo "Error during compilation. Please examine and cleanup if needed:"
    echo "Directory: $tmpdir/new/$maindir"
    echo "     File: $mainbase.tex"
    # Don't clean up to let the user diagnose.
    exit 1
fi

if test -n "$output" ; then
    abs_pdffile="$PWD/$pdffile"
    (cd "$initial_dir" && mv "$abs_pdffile" "$output")
    echo "Output written on $output"
elif [ -f "$pdffile" ]; then
    new_pdffile="$tmpdir"/"$pdffile"
    mv "$pdffile" "$new_pdffile"
    pdffile="$new_pdffile"
fi

# Change directory so nothing will keep us from cleaning
cd "$initial_dir"

if test "$view" = 1  || test "$view" = maybe  && test -z "$output" ; then
    "$PDFVIEWER" "$pdffile"
fi

case "$cleanup" in
    "all")
	verbose "Cleaning-up result"
	rm -fr "$tmpdir"
	verbose_done
	;;
    "keeppdf")
	verbose "Cleaning-up all but pdf (kept in $pdffile)"
	rm -fr "$tmpdir"/old "$tmpdir"/new
	verbose_done
	;;
    "none")
	verbose_say "Generated files kept in $tmpdir/"
	;;
esac


==> graph/Makefile <==
GNUPLOT ?= gnuplot
GNUPLOT_VERSION = gnuplot 5.2 patchlevel 7

scripts := $(wildcard scripts/*.gpl)

.PHONY: graphs
graphs: check_gnuplot
	for s in $(scripts); do \
	  echo $$s; \
	  $(GNUPLOT) $$s;\
	done

	for s in $(wildcard *.eps); do \
		epstool --copy --bbox $$s tmp.eps; \
		mv tmp.eps $$s; \
	done

.PHONY: clean
clean:
	$(RM) *.eps
	$(RM) *.pdf

.PHONY: check_gnuplot
check_gnuplot:
	[ "x$(shell gnuplot --version)" == "x$(GNUPLOT_VERSION)" ]

